Twisted hyperbolic van der Waals crystals for full Stokes mid-infrared polarization detection

Investigating the polarization properties of light in the mid-infrared (mid-IR) spectrum is crucial for molecular sensing, biomedical diagnostics, and IR imaging system technologies. Traditional methods, limited by bulky size and intricate fabrication, utilize large rotating optics for full Stokes polarization detection, impeding miniaturization and accuracy. Van der Waals materials (vdW) based devices can address these challenges due to their lithography-free fabrication, ease of integration with chip-scale platforms and room-temperature operation. This study introduces a chip-integrated polarimeter device leveraging the in-plane biaxial hyperbolic vdW crystal properties for mid-infrared light manipulation. The spatial division measurement scheme incorporates six meticulously designed linear and circular polarization filters, achieving high extinction ratios exceeding 30 dB and transmittance surpassing 50%, with fabrication tolerance of film thickness up to 100 nm. The proposed device represents a significant advancement in polarimetric detection, providing a compact, cost-effective solution and opens new avenues for on-chip mid-IR polarimetric detection in next-generation ultra-compact optical systems.

==> biblio.tex <==
\addcontentsline{toc}{section}{Bibliography}
\bibliographystyle{unsrt}
\bibliography{ref.bib}
